STL-Based Synthesis of Feedback Controllers Using Reinforcement Learning

Deep Reinforcement Learning (DRL) has the potential to be used for synthesizing feedback controllers (agents) for various complex systems with unknown dynamics. These systems are expected to satisfy diverse safety and liveness properties best captured using temporal logic. In RL, the reward function plays a crucial role in specifying the desired behaviour of these agents. However, the problem of designing the reward function for an RL agent to satisfy complex temporal logic specifications has received limited attention in the literature. To address this, we provide a systematic way of generating rewards in real-time by using the quantitative semantics of Signal Temporal Logic (STL), a widely used temporal logic to specify the behaviour of cyber-physical systems. We propose a new quantitative semantics for STL having several desirable properties, making it suitable for reward generation. We evaluate our STL-based reinforcement learning mechanism on several complex continuous control benchmarks and compare our STL semantics with those available in the literature in terms of their efficacy in synthesizing the controller agent. Experimental results establish our new semantics to be the most suitable for synthesizing feedback controllers for complex continuous dynamical systems through reinforcement learning.

==> Related_Work.tex <==

\section{Related Work}

Temporal Logic has been extremely popular in the area of CPSs, where desirable behaviour has been encoded for verification using LTL~\cite{Pnueli77}, MTL~\cite{Koymans05}, and STL~\cite{donze10a,jaksic18}. Recently, several papers address the controller synthesis problem  using the temporal logic~\cite{raman15,Duggirala16,Pant18}. 
However, unlike our work, these papers assume that the model of the system under control is available for controller synthesis.


% There are different approaches to controller synthesis.
In our controller synthesis methodology, we rely on gradient-based optimization for finding the weights of the neural network controller.
% Convex optimization is difficult with the classical semantics of STL in~\cite{donze10a} since it is non-convex. 
Heuristic based approaches such as simulated annealing has been proposed in~\cite{abbas12}. These algorithms require many user-defined parameters in advance. Another approach is encode STL-constraints as MILP~\cite{Saha16}. However, MILP solvers suffer from the issue of scalability.
%The most recent approach has been to use gradients of smooth semantics of STL~\cite{lse,Pant17}.

% There have been many recent works on proposing different STL semantics to address the shortcomings of the classical semantics.
% In~\cite{lse}-\cite{Pant17}, the authors have proposed a log-sum-exponential based semantics for computation of robustness metric. In~\cite{varnai20}, the authors propose a softmax based semantics for robustness computation. In~\cite{agm}, authors present a arithmetic-geometric mean based semantics for robustness computation.

In RL domain, reward shaping has been a popular way to synthesize controllers.
Earlier approaches to Reward shaping has been via potential-based function~\cite{ng99}, inverse reinforcement learning~\cite{Abbeel04}, etc.
In~\cite{Aksaray16}, the authors propose to use the robustness with respect to an STL formula as reward function for Q-Learning. 
The idea of controller synthesis using Truncated LTL as rewards has been explored in~\cite{belta17} and with STL in~\cite{Balakrishnan19}.
Of late, there have been many works in the area of controller synthesis that guides the synthesis using a set of good trajectories ~\cite{levine13}. This search can be both under known dynamics~\cite{zhang16} or unknown dynamics~\cite{levine14}. 



==> comparison.tex <==
\section{Comparison}
\label{compare}
In~\cite{Balakrishnan19}, the authors use STL specification to shape the rewards.
For the CartPole example, we trained the DDQN agent with both nominal reward as well as with online STL robustness as shown in Figure~\ref{fig:comp1}. 

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\columnwidth]{fig/dqn_cp_episode_reward_both.pdf} % Here comes the figure file path
    \caption{Comparison}
    \label{fig:comp1}
\end{figure}


Mention the following
\begin{itemize}
    \item low dimentionality of our solution
    \item single-step reward computation vs BHNR metric used by them.
    \item Suitability to continuous control
    \item Training time comparison
    \item comparison of policies
\end{itemize}

\subsection{W.r.t normalisation}
Now we show the benefit of normalisation using the pendulum example. Using the classical STL robustness, we observe that the reward generation is not uniform, i.e., there is not a single maxima (and hence non-convex). So, the trained policy once picks a direction of maxima will go on in the direction eventually achieving it.  
Note that there is a slight difference in the values of the two maximas.
However, it will never be the case that policy will move from one maxima to the other maxima as there is lesser reward in the path joining the two maximas.
\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\columnwidth]{fig/pendulum_anamoly.pdf} % Here comes the figure file path
     \caption{Issue in reward generation with classical STL robustness}
    \label{fig:pend_anamoly}
\end{figure}


In case of the pendulum example, the reward at each step lies in the range [-8,1] with the domains $\theta \in [-1,1]$, $\dot{\theta} \in [-8,8]$ and $u \in [-2,2]$.

Lets consider when the pendulum is in stable positions i.e. when $\dot{\theta}$ and $u$ are both close to zero and the reward depends solely on $\theta$. There ae only two such configurations - one when pendulum is upright and the other when pendulum is downward as shown in Figure~\ref{fig:pend_anamoly1} and Figure~\ref{fig:pend_anamoly2}. This two positions correspond to the two maximas in Figure~\ref{fig:pend_anamoly}.
In the downward equilibrim, the reward at each step is roughly around $-1.9$ while in upward equilibrium, the reward at each step is around $-0.6$. Apart the these two configurations, the reward takes high negative values around $-8$ in other states due to higher values of $\dot{\theta}$ (say,in horizontal position).


\begin{figure}[!htbp]
    \centering
     \includegraphics[width=\columnwidth]{fig/pend_down_wn.png}
     \caption{Issue in reward generation with classical STL robustness}
    \label{fig:pend_anamoly1}
\end{figure}

\begin{figure}[!htbp]
    \centering
    \includegraphics[width=\columnwidth]{fig/pend_up_wn.png}
     \caption{Issue in reward generation with classical STL robustness}
    \label{fig:pend_anamoly2}
\end{figure}

The above anomaly is due to the non-convexity of the reward function. So, we make the reward generation function convex which eventually gives us function with single maxima enabling us to always learn the optimal policy. This transformation is achieved via normalisation.
In the above description, convexity refers to the class of problems - the function however is concave and can be converted to convex function.

Using normalisation, we will always get higher reward as we move the pendulum upwards. The above discussion leads us to following theorem.

\begin{theorem}
Consider a specification $\phi$ which is consists of the set of predicates $\kappa_1,....\kappa_n$. If there exists different size domains of predicate $\kappa_i$ for $i \in [1,n]$, i.e., $\mathcal{D}_{\kappa_i} \neq \mathcal{D}_{\kappa_j}$ for some $i,j \in [1,n]$, then using the reward based on classical robustness $\rho$ for learning might give us a sub-optimal controller. Using normalised robustness $\rho^n$ would give us an optimal controller in such cases.
\end{theorem}

% \par Corollary:
% For the above theorem, if the specification consists of conjunction of predicates, then 
% following always holds:
% \begin{itemize}
%     \item $\rho(\phi) = \underset{i}{\mathtt{min}} (\mathtt{min} (\mathcal{D}_{\kappa_i}^-))$ when robustness is negative 
%     \item $\rho(\phi) = \underset{i}{\mathtt{min}}( \mathtt{max} (\mathcal{D}_{\kappa_i}^+))$ when robustness is positive 
% \end{itemize}
% where $\mathcal{D}^-$ and $\mathcal{D}^+$ represents the negative and positive values in the domain. Here the outer min is used as per the robustness semantics for conjunction operator.

% Let us consider an atomic specification $\phi$ and denote its predicate using $\kappa$. We define the domain $\mathcal{D}_{\kappa}$ of a  predicate $\kappa$ as the union of the domain of variables in the predicates. We define the length of a domain of a predicate $\kappa$ as the absolute difference (L1-norm) of the maximum and minimum value of the domain of $\kappa$ , i.e.
% $length(\mathcal{D}_{\kappa}) = |max(\mathcal{D}_{\kappa})-min(\mathcal{D}_{\kappa})|$.





% \begin{figure}[!htbp]
%     \includegraphics[width=.23\textwidth]{fig/ddpg_pend_episode_reward_without_norm.pdf}\hfill
%     \includegraphics[width=.23\textwidth]{fig/ddpg_pend_episode_reward_STL_norm.pdf}
%   \caption{Comparison w.r.t normalisation}
%     \label{fig:comp2}
% \end{figure}

% In the figure~\ref{fig:comp2}, we show the plots for two experiments. In the first experiment, we trained the policy using the non-normalised version of the formulae (left plot) and in the second experiment, we used the normalised formulae (right plot). 
